Resolutions for representations of reductive p-adic groups via their buildings

Schneider-Stuhler and Vigneras have used cosheaves on the affine Bruhat-Tits building to construct natural finite type projective resolutions for admissible representations of reductive p-adic groups in characteristic not equal to p. We use a system of idempotent endomorphisms of a representation with certain properties to construct a cosheaf and a sheaf on the building. We establish that these are acyclic and compute homology and cohomology with these coefficients. This implies Bernstein's result that certain subcategories of the category of representations are Serre subcategories. Furthermore, we also get results for convex subcomplexes of the building. Following work of Korman, this leads to trace formulas for admissible representations.

==> Resolutions_1_.tex <==
\newbox\ASYbox
\newdimen\ASYdimen
\def\ASYbase#1#2{\setbox\ASYbox=\hbox{#1}\ASYdimen=\ht\ASYbox%
\setbox\ASYbox=\hbox{#2}\lower\ASYdimen\box\ASYbox}
\def\ASYalign(#1,#2)(#3,#4)#5#6{\leavevmode%
\setbox\ASYbox=\hbox{#6}%
\setbox\ASYbox\hbox{\ASYdimen=\ht\ASYbox%
\advance\ASYdimen by\dp\ASYbox\kern#3\wd\ASYbox\raise#4\ASYdimen\box\ASYbox}%
\put(#1,#2){%
\special{pdf:q #5 0 0 cm}\wd\ASYbox 0pt\dp\ASYbox 0pt\ht\ASYbox 0pt%
\box\ASYbox%
\special{pdf:Q}%
}}
\def\ASYraw#1{#1}
\setlength{\unitlength}{1pt}
\includegraphics{Resolutions_1_0.pdf}%
\special{pdf:q}%
\begin{picture}( 341.432399, 170.716199)%
\special{pdf:\ASYraw{
 -340.156811 0.000000 m
 0.000000 0.000000 l
 0.000000 170.078405 l
 -340.156811 170.078405 l
 -340.156811 0.000000 l
h
W n
}%
}%
\end{picture}%
\kern -341.432399pt%
\special{pdf:Q}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.000000}{12.000000}\selectfont
\usefont{OT1}{cmr}{m}{n}%
\ASYalign(-298.753349,26.557663)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{\(\sigma\)}
\ASYalign(-258.212929,68.659330)(0.000000,0.000000){1.000000 0.000000 0.000000 1.000000}{\(\tau\)}
\ASYalign(-279.120986,51.745598)(-0.500000,-0.500000){1.000000 0.000000 0.000000 1.000000}{\(\Hull(\sigma,\tau)\)}
\ASYalign(-110.965530,136.071359)(-0.500000,0.000000){1.000000 0.000000 0.000000 1.000000}{\(x\)}
\ASYalign(-85.358100,41.342120)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{\(\omega\)}
\ASYalign(-102.429720,88.706739)(-0.500000,-0.500000){1.000000 0.000000 0.000000 1.000000}{\(\Hull(\omega,x)\)}
\ASYalign(-187.787819,159.617772)(-0.500000,-0.781250){1.000000 0.000000 0.000000 1.000000}{convex subcomplex}


==> Resolutions_2_.tex <==
\newbox\ASYbox
\newdimen\ASYdimen
\def\ASYbase#1#2{\setbox\ASYbox=\hbox{#1}\ASYdimen=\ht\ASYbox%
\setbox\ASYbox=\hbox{#2}\lower\ASYdimen\box\ASYbox}
\def\ASYalign(#1,#2)(#3,#4)#5#6{\leavevmode%
\setbox\ASYbox=\hbox{#6}%
\setbox\ASYbox\hbox{\ASYdimen=\ht\ASYbox%
\advance\ASYdimen by\dp\ASYbox\kern#3\wd\ASYbox\raise#4\ASYdimen\box\ASYbox}%
\put(#1,#2){%
\special{pdf:q #5 0 0 cm}\wd\ASYbox 0pt\dp\ASYbox 0pt\ht\ASYbox 0pt%
\box\ASYbox%
\special{pdf:Q}%
}}
\def\ASYraw#1{#1}
\setlength{\unitlength}{1pt}
\includegraphics{Resolutions_2_0.pdf}%
\special{pdf:q}%
\begin{picture}( 199.168899, 85.358100)%
\special{pdf:\ASYraw{
 -198.424806 0.000000 m
 0.000000 0.000000 l
 0.000000 85.039203 l
 -198.424806 85.039203 l
 -198.424806 0.000000 l
h
W n
}%
}%
\end{picture}%
\kern -199.168899pt%
\special{pdf:Q}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.000000}{12.000000}\selectfont
\usefont{OT1}{cmr}{m}{n}%
\ASYalign(-179.958650,31.019927)(-1.000000,-1.000000){1.000000 0.000000 0.000000 1.000000}{\(\tau\)}
\ASYalign(-26.323425,72.239619)(0.000000,0.000000){1.000000 0.000000 0.000000 1.000000}{\(x\)}
\ASYalign(-170.736116,37.205072)(-0.500000,-0.500000){1.000000 0.000000 0.000000 1.000000}{\(\sigma\)}
\ASYalign(-99.584450,73.121594)(-0.500000,0.250000){1.000000 0.000000 0.000000 1.000000}{\(\mathcal{H}(\tau,x)\)}


==> Resolutions_3_.tex <==
\newbox\ASYbox
\newdimen\ASYdimen
\def\ASYbase#1#2{\setbox\ASYbox=\hbox{#1}\ASYdimen=\ht\ASYbox%
\setbox\ASYbox=\hbox{#2}\lower\ASYdimen\box\ASYbox}
\def\ASYalign(#1,#2)(#3,#4)#5#6{\leavevmode%
\setbox\ASYbox=\hbox{#6}%
\setbox\ASYbox\hbox{\ASYdimen=\ht\ASYbox%
\advance\ASYdimen by\dp\ASYbox\kern#3\wd\ASYbox\raise#4\ASYdimen\box\ASYbox}%
\put(#1,#2){%
\special{pdf:q #5 0 0 cm}\wd\ASYbox 0pt\dp\ASYbox 0pt\ht\ASYbox 0pt%
\box\ASYbox%
\special{pdf:Q}%
}}
\def\ASYraw#1{#1}
\setlength{\unitlength}{1pt}
\includegraphics{Resolutions_3_0.pdf}%
\special{pdf:q}%
\begin{picture}( 341.432399, 170.716199)%
\special{pdf:\ASYraw{
 -340.156811 0.000000 m
 0.000000 0.000000 l
 0.000000 170.078405 l
 -340.156811 170.078405 l
 -340.156811 0.000000 l
h
W n
}%
}%
\end{picture}%
\kern -341.432399pt%
\special{pdf:Q}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.000000}{12.000000}\selectfont
\usefont{OT1}{cmr}{m}{n}%
\ASYalign(-119.501340,91.717989)(-0.500000,0.000000){1.000000 0.000000 0.000000 1.000000}{$x$}
\ASYalign(-59.750670,76.933533)(-0.500000,0.000000){1.000000 0.000000 0.000000 1.000000}{$\tau$}
\ASYalign(-93.893910,91.717989)(-0.500000,0.250000){1.000000 0.000000 0.000000 1.000000}{$\mathcal{H}(x,\tau)$}
\ASYalign(-73.407966,130.048859)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{$\tau$}
\ASYalign(-42.679050,106.502446)(-0.500000,0.218750){1.000000 0.000000 0.000000 1.000000}{problems}
\ASYalign(-273.145919,3.011250)(-0.500000,0.000000){1.000000 0.000000 0.000000 1.000000}{admissible}
\ASYalign(-85.358100,3.011250)(-0.500000,0.000000){1.000000 0.000000 0.000000 1.000000}{not admissible}


==> Resolutions_4_.tex <==
\newbox\ASYbox
\newdimen\ASYdimen
\def\ASYbase#1#2{\setbox\ASYbox=\hbox{#1}\ASYdimen=\ht\ASYbox%
\setbox\ASYbox=\hbox{#2}\lower\ASYdimen\box\ASYbox}
\def\ASYalign(#1,#2)(#3,#4)#5#6{\leavevmode%
\setbox\ASYbox=\hbox{#6}%
\setbox\ASYbox\hbox{\ASYdimen=\ht\ASYbox%
\advance\ASYdimen by\dp\ASYbox\kern#3\wd\ASYbox\raise#4\ASYdimen\box\ASYbox}%
\put(#1,#2){%
\special{pdf:q #5 0 0 cm}\wd\ASYbox 0pt\dp\ASYbox 0pt\ht\ASYbox 0pt%
\box\ASYbox%
\special{pdf:Q}%
}}
\def\ASYraw#1{#1}
\setlength{\unitlength}{1pt}
\includegraphics{Resolutions_4_0.pdf}%
\special{pdf:q}%
\begin{picture}( 341.432399, 170.716199)%
\special{pdf:\ASYraw{
 -340.156811 0.000000 m
 0.000000 0.000000 l
 0.000000 170.078405 l
 -340.156811 170.078405 l
 -340.156811 0.000000 l
h
W n
}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.000000}{12.000000}\selectfont
\usefont{OT1}{cmr}{m}{n}%
\ASYalign(-179.252009,11.773207)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{$x$}
\ASYalign(-190.799069,29.568913)(-1.000000,-0.188889){1.000000 0.000000 0.000000 1.000000}{$y$}
\ASYalign(-170.716199,26.557663)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{$z$}
\ASYalign(-247.538489,41.342120)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{$a$}
\ASYalign(-236.873404,57.008551)(0.000000,-1.000000){1.000000 0.000000 0.000000 1.000000}{$b$}
\ASYalign(-258.203574,57.008551)(-1.000000,-1.000000){1.000000 0.000000 0.000000 1.000000}{$c$}
\ASYalign(-117.372064,61.267101)(0.000000,0.218750){1.000000 0.000000 0.000000 1.000000}{second forbidden region}
\ASYalign(-247.538489,162.629022)(-0.500000,-0.281250){1.000000 0.000000 0.000000 1.000000}{first forbidden region}
\end{picture}%
\kern -341.432399pt%
\special{pdf:Q}%


==> Resolutions_5_.tex <==
\newbox\ASYbox
\newdimen\ASYdimen
\def\ASYbase#1#2{\setbox\ASYbox=\hbox{#1}\ASYdimen=\ht\ASYbox%
\setbox\ASYbox=\hbox{#2}\lower\ASYdimen\box\ASYbox}
\def\ASYalign(#1,#2)(#3,#4)#5#6{\leavevmode%
\setbox\ASYbox=\hbox{#6}%
\setbox\ASYbox\hbox{\ASYdimen=\ht\ASYbox%
\advance\ASYdimen by\dp\ASYbox\kern#3\wd\ASYbox\raise#4\ASYdimen\box\ASYbox}%
\put(#1,#2){%
\special{pdf:q #5 0 0 cm}\wd\ASYbox 0pt\dp\ASYbox 0pt\ht\ASYbox 0pt%
\box\ASYbox%
\special{pdf:Q}%
}}
\def\ASYraw#1{#1}
\setlength{\unitlength}{1pt}
\includegraphics{Resolutions_5_0.pdf}%
\special{pdf:q}%
\begin{picture}( 318.670239, 119.501340)%
\special{pdf:\ASYraw{
 -317.479690 0.000000 m
 0.000000 0.000000 l
 0.000000 119.054884 l
 -317.479690 119.054884 l
 -317.479690 0.000000 l
h
W n
}%
}%
\end{picture}%
\kern -318.670239pt%
\special{pdf:Q}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.000000}{12.000000}\selectfont
\usefont{OT1}{cmr}{m}{n}%
\ASYalign(-271.007289,44.279608)(-1.000000,-0.741629){1.000000 0.000000 0.000000 1.000000}{\(\tau=\tau_0\)}
\ASYalign(-39.833780,101.165731)(-0.500000,0.000000){1.000000 0.000000 0.000000 1.000000}{\(\sigma\)}
\ASYalign(-199.168899,101.165731)(-0.500000,0.000000){1.000000 0.000000 0.000000 1.000000}{\(\omega\)}
\ASYalign(-258.919569,52.158394)(-0.500000,-0.241629){1.000000 0.000000 0.000000 1.000000}{\(\tau_1\)}
\ASYalign(-248.961124,46.408883)(-0.500000,-0.241629){1.000000 0.000000 0.000000 1.000000}{\(\tau_2\)}
\ASYalign(-239.002679,40.659372)(-0.500000,-0.241629){1.000000 0.000000 0.000000 1.000000}{\(\tau_3\)}
\ASYalign(-229.044234,46.408883)(-0.500000,-0.241629){1.000000 0.000000 0.000000 1.000000}{\(\tau_4\)}
\ASYalign(-219.085789,52.158394)(-0.500000,-0.241629){1.000000 0.000000 0.000000 1.000000}{\(\tau_5\)}
\ASYalign(-219.085789,63.657416)(-0.500000,-0.241629){1.000000 0.000000 0.000000 1.000000}{\(\tau_6\)}
\ASYalign(-219.085789,75.156438)(-0.500000,-0.241629){1.000000 0.000000 0.000000 1.000000}{\(\tau_7\)}
\ASYalign(-209.127344,80.905949)(-0.500000,-0.241629){1.000000 0.000000 0.000000 1.000000}{\(\tau_8\)}
\ASYalign(-199.168899,86.655460)(-0.500000,-0.241629){1.000000 0.000000 0.000000 1.000000}{\(\tau_9\)}
\ASYalign(-231.173509,83.035224)(-1.000000,0.250000){1.000000 0.000000 0.000000 1.000000}{\(\tau_7\subseteq\mathcal{H}(\tau_6,\omega)\)}
\ASYalign(-139.418229,60.646166)(-0.500000,-0.750000){1.000000 0.000000 0.000000 1.000000}{\(\omega\subseteq\mathcal{H}(\tau_6,\sigma)\)}


==> Resolutions_6_.tex <==
\newbox\ASYbox
\newdimen\ASYdimen
\def\ASYbase#1#2{\setbox\ASYbox=\hbox{#1}\ASYdimen=\ht\ASYbox%
\setbox\ASYbox=\hbox{#2}\lower\ASYdimen\box\ASYbox}
\def\ASYalign(#1,#2)(#3,#4)#5#6{\leavevmode%
\setbox\ASYbox=\hbox{#6}%
\setbox\ASYbox\hbox{\ASYdimen=\ht\ASYbox%
\advance\ASYdimen by\dp\ASYbox\kern#3\wd\ASYbox\raise#4\ASYdimen\box\ASYbox}%
\put(#1,#2){%
\special{pdf:q #5 0 0 cm}\wd\ASYbox 0pt\dp\ASYbox 0pt\ht\ASYbox 0pt%
\box\ASYbox%
\special{pdf:Q}%
}}
\def\ASYraw#1{#1}
\setlength{\unitlength}{1pt}
\includegraphics{Resolutions_6_0.pdf}%
\special{pdf:q}%
\begin{picture}( 199.168899, 85.358100)%
\special{pdf:\ASYraw{
 -198.424806 0.000000 m
 0.000000 0.000000 l
 0.000000 85.039203 l
 -198.424806 85.039203 l
 -198.424806 0.000000 l
h
W n
}%
}%
\end{picture}%
\kern -199.168899pt%
\special{pdf:Q}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.000000}{12.000000}\selectfont
\usefont{OT1}{cmr}{m}{n}%
\ASYalign(-179.958650,31.019927)(-1.000000,-1.000000){1.000000 0.000000 0.000000 1.000000}{\(\tau\)}
\ASYalign(-42.679050,73.121594)(-0.500000,0.000000){1.000000 0.000000 0.000000 1.000000}{\(\sigma\)}
\ASYalign(-170.716199,17.817572)(-0.500000,-0.741629){1.000000 0.000000 0.000000 1.000000}{\(z_0\)}
\ASYalign(-142.263499,17.817572)(-0.500000,-0.741629){1.000000 0.000000 0.000000 1.000000}{\(z_1\)}
\ASYalign(-113.810800,17.817572)(-0.500000,-0.741629){1.000000 0.000000 0.000000 1.000000}{\(z_2\)}
\ASYalign(-98.432094,42.687551)(-0.292893,-0.741629){1.000000 0.000000 0.000000 1.000000}{\(z_3\)}
\ASYalign(-71.131750,42.458333)(-0.500000,-0.741629){1.000000 0.000000 0.000000 1.000000}{\(z_4\)}
\ASYalign(-40.549775,43.340308)(0.000000,-0.688889){1.000000 0.000000 0.000000 1.000000}{\(z_5=y\)}
\ASYalign(-128.037150,67.099094)(-0.500000,-0.750000){1.000000 0.000000 0.000000 1.000000}{\(\mathcal{H}(\sigma,\tau)\)}

